Reference Network and Localization Architecture for Smart Manufacturing based on 5G

5G promises to shift Industry 4.0 to the next level by allowing flexible production. However, many communication standards are used throughout a production site, which will stay so in the foreseeable future. Furthermore, localization of assets will be equally valuable in order to get to a higher level of automation. This paper proposes a reference architecture for a convergent localization and communication network for smart manufacturing that combines 5G with other existing technologies and focuses on high-mix low-volume application, in particular at small and medium-sized enterprises. The architecture is derived from a set of functional requirements, and we describe different views on this architecture to show how the requirements can be fulfilled. It connects private and public mobile networks with local networking technologies to achieve a flexible setup addressing many industrial use cases.

==> 2022-04-01 SysInt22 Reference Networking and Localization Architecture submitted/acronyms.tex <==
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{itu}{ITU}{International Telecommunication Union}
\newacronym{iiot}{IIoT}{Industrial Internet of Things}
\newacronym{mc-ss}{MC-SS}{multi-carrier spread spectrum}
\newacronym{mccdma}{MC-CDMA}{multi-carrier code division multiple access}
\newacronym{mmtc}{mMTC}{massive machine type communications}
\newacronym{urllc}{uRLLC}{ultra-reliable and low latency communications}
\newacronym{embb}{eMBB}{enhanced mobile broadband}
\newacronym{sdn}{SDN}{software-defined network}
\newacronym{rru}{RRU}{remote radio unit}
\newacronym{bs}{BS}{base station}
\newacronym{sgw}{S-Gw}{serving gateway}
\newacronym{pgw}{P-Gw}{packet data network gateway}
\newacronym{up}{UP}{user plane}
\newacronym{upf}{UPF}{user plane function}
\newacronym{cp}{CP}{control plane}
\newacronym{ausf}{AUSF}{authentication server function}
\newacronym{udm}{UDM}{user data management}
\newacronym{hss}{HSS}{home subscriber server}
\newacronym{smf}{SMF}{session management function}
\newacronym{mme}{MME}{mobility management entity}
\newacronym{pcf}{PCF}{policy control function}
\newacronym{ap}{AP}{aggregation point}
\newacronym{prp}{PRP}{parallel redundancy protocol}
\newacronym{tcp}{TCP}{transmission control protocol}
\newacronym{api}{API}{application programming interface}
\newacronym{ovs}{OvS}{open vSwitch}
\newacronym{wlan}{WLAN}{wireless local area network}
\newacronym{wan}{WAN}{wide area network}
\newacronym{lpwan}{LPWAN}{low-power wide area network}
\newacronym{ble}{BLE}{Bluetooth low energy}
\newacronym{3gpp}{3GPP}{3rd Generation Partnership Project}
\newacronym{itur}{ITU-R}{International Telecommunication Union Radiocommunication Sector}
\newacronym{qos}{QoS}{quality of service}
\newacronym{nbiot}{NB-IoT}{narrow-band IoT}
\newacronym{ec}{EC}{edge cloud}
\newacronym{nfv}{NFV}{network function virtualization}
\newacronym{iira}{IIRA}{Industrial Internet Reference Architecture}
\newacronym{iic}{IIC}{Industrial Internet Consortium}
\newacronym{rami}{RAMI~4.0}{Reference Architectural Model of Industry 4.0}
\newacronym{mes}{MES}{manufacturing execution system}
\newacronym{erp}{ERP}{enterprise resource planning}
\newacronym{ngmn}{NGMN}{Next Generation Mobile Networks}
\newacronym{agv}{AGV}{automated guided vehicle}
\newacronym{agc}{AGC}{automated guided cart}
\newacronym{slam}{slam}{simultaneous locating and mapping}
\newacronym{mno}{MNO}{mobile network operator}
\newacronym{plc}{PLC}{programmable logic controller}
\newacronym{epc}{EPC}{evolved packet core}
\newacronym{indot}{ind. OT}{industrial operation technology}
\newacronym{ot}{OT}{operation technology}
\newacronym{ict}{ICT}{information and communication technology}
\newacronym{cmtc}{cMTC}{critical Machine Type Communications}
\newacronym{nr}{NR}{New Radio}
\newacronym{das}{DAS}{distributed antenna system}
\newacronym{hmi}{HMI}{human machine interface}
\newacronym{etsi}{ETSI}{European Telecommunications Standards Institute}
\newacronym{mec}{MEC}{multi-access edge computing}
\newacronym{acia}{5G ACIA}{5G Alliance for Connected Industries and Automation}
\newacronym{ue}{UE}{equipment}
\newacronym{hmlv}{HMLV}{high mix, low volume}
\newacronym{sme}{SME}{small and medium-sized enterprise}
\newacronym{5g}{5G}{5th generation of mobile communications}
\newacronym{cpps}{CPPS}{cyber-physical production system}
\newacronym{m2m}{M2M}{machine-to-machine}
\newacronym{roi}{ROI}{return on invest}
\newacronym{it}{IT}{information technology}
\newacronym{e2e}{E2E}{end-to-end}
\newacronym{eap}{EAP}{extensible authentication protocol}
\newacronym{aka}{5G AKA}{5G authentication and key agreement}
